Nature of the current-induced insulator-to-metal transition in Ca$_2$RuO$_4$ as revealed by transport-ARPES

The Mott insulator Ca$_2$RuO$_4$ exhibits a rare insulator-to-metal transition (IMT) induced by DC current. While structural changes associated with this transition have been tracked by neutron diffraction, Raman scattering, and x-ray spectroscopy, work on elucidating the response of the electronic degrees of freedom is still in progress. Here we unveil the current-induced modifications of the electronic states of Ca$_2$RuO$_4$ by employing angle-resolved photoemission spectroscopy (ARPES) in conjunction with four-probe transport. Two main effects emerge: a clear reduction of the Mott gap and a modification in the dispersion of the Ru-bands. The changes in dispersion occur exclusively along the $XM$ high-symmetry direction, parallel to the $b$-axis where the greatest in-plane lattice change occurs. These experimental observations, together with dynamical mean-field theory (DMFT) calculations simulated from the current-induced structural distortions, indicate the intimate interplay of lattice and orbital-dependent electronic response in the current-driven IMT. Furthermore, based on a free energy analysis, we demonstrate that the current-induced phase, albeit thermodynamically equivalent, is electronically distinct from the high-temperature zero-current metallic phase. Our results provide insight into the elusive nature of the current-induced IMT of Ca$_2$RuO$_4$ and advance the challenging, yet powerful, technique of transport-ARPES.

==> append.tex <==
\chapter*{Appendix}

\usepackage{graphicx}

\begin{appendices}

\section{Characterization on CRO crystals}\label{secA1}

\begin{figure}[h]%
\centering
\includegraphics[width=0.999\textwidth]{characterization.pdf}
\caption{(a) SQUID magnetometry along the high symmetry directions of the crystal. (b) X-ray Laue diffraction pattern showing crystal is aligned to a high symmetry direction. (c) Single crystal diffraction determination of high-symmetry directions. The data is taken from (d) 0kl (e) h0l and (f) hk0 planes.}\label{sup1}
\end{figure}

Magnetometry and single crystal diffraction is used to confirm alignment along a specific axis, since the principal axes are indistinguishable in x-ray Laue diffraction, as shown in Fig.~\ref{sup1}. When the crystal is aligned along the $a$-axis, a peak at $T_{\mathrm{N}} = 110$~K is observed in magnetization, however, this peak disappears when the crystal is aligned along the $b$-axis.

\section{ARPES on CRO}\label{secA2}

\begin{figure}[h]%
\centering
\includegraphics[width=0.999\textwidth]{photonEdep.pdf}
\caption{(a-f) Photon energy dependence of the ruthenium bands taken with $\sigma$-polarized light. }\label{sup2}
\end{figure}

In order to carefully discriminate the current-induced effects predicted by the DMFT, it is crucial to be at the correct photon energy, or $k_{z}$. A photon energy dependence of the electronic structure at the $XM$ line at the Brillouin zone edge is shown in Fig.~\ref{sup2}. The dispersive feature is most prominent at a photon energy of 74~eV. Note, Fig.~\ref{sup2}e and j are taken with different statistics.

\begin{figure}[h]%
\centering
\includegraphics[width=0.999\textwidth]{LH.pdf}
\caption{Data taken with $\pi$-polarized light and with the analyzer slit aligned along the (a - d) $b$-axis and (e - g) $a$-axis. (a, b) $XM$ high symmetry cuts in the (a) S- and (b) L*-phases. (c) Corresponding EDCs integrated over the Brilloun zone. (d) Fermi surface in L* phase. (e, f) YM high symmetry cuts in the (e) S- and (f) L*-phases. (g) Corresponding EDCs integrated over the Brilloun zone.}\label{sup3}
\end{figure}

While different atomic orbitals are sensitive to orthogonal polarizations of light, the clearest picture of the electron band structure of CRO is given by $\sigma$-polarized light that is in our experimental geometry sensitive to the $d_{xy}$ and $d_{yz}$ orbitals. Meanwhile, $\pi$-polarized light is most sensitive to the $d_{xz}$ bands, which are not fully populated in the insulating state. This results in spectra where features are difficult to discern, however for completion we have included the cuts along the Brillouin zone edge taken with $\pi$-polarized light in Fig.~\ref{sup3}. Note, the asymmetry of the Fermi surfaces indicating the presence of strong matrix element effects.

\begin{figure}[h]%
\centering
\includegraphics[width=0.67\textwidth]{GammaCuts.pdf}
\caption{Cuts through the $\Gamma$ point. (a - g) Cuts along $\Gamma X$ in (b, c) $\sigma$- and (e, f) $\pi$-polarization in the (b, e) S*- and (c, f) L*-phases. (d, g) Accompanying EDCs, integrated across the $X \Gamma X$ cut, between the equilibrium and non-equilibrium phases. (h - n) Cuts along $\Gamma Y$ in (i ,j) $\sigma$- and (l, m) $\pi$-polarization in the (i ,l) S*- and (j, m) L*-phases. (k, n) Accompanying EDCs, integrated across the $X \Gamma X$ cut, between the equilibrium and non-equilibrium phases. (a, h) Only MDCs for $\sigma$-polarization data (b, i) without and (c, j) with current, where changes seemingly happen, is shown. The current is applied along the $b$-axis, parallel to the $\Gamma Y$ direction.}\label{sup7}
\end{figure}

To further compound that changes only occur along the $XM$ cut, cuts through the $\Gamma$-point were taken and are shown in Fig.~\ref{sup7}. Following the previous discussion, minimal changes can be seen in $\pi$-polarized and along the $\Gamma X$ high symmetry direction, perpendicular to the current flow. On the other hand, the $\Gamma Y$ cuts seem to exhibit changes however, upon closer inspection of the EDCs and MDCs shown in Fig.~\ref{sup7}a, d, g, h, k, and n, no large differences are observed. The most significant change occurs along $\Gamma Y$, where an increase in spectral weight is seen at the edge of the Brillouin zone at the Y points.

%This corresponds with the shifted spectral weight towards Fermi level from the higher to lower energy Ru-band seen in Fig.~\ref{fig4}.

\begin{figure}[h]%
\centering
\includegraphics[width=0.999\textwidth]{chargeage.pdf}
\caption{EDCs (a) for different sizes of the beamline exit slit and (b) at the beginning of the experiment and a week later, integrated along the $XM$ cut, indicating that minimal aging and charging affects take place.}\label{sup4}
\end{figure}

Given the insulating nature of the crystal, sample charging affecting the measured spectra can be an experimental obstacle. The extent of charging can be recorded by changing the flux of incident photons on the sample. By modifying the size of the beamline exit slit, we see in Fig.~\ref{sup4}a that some charging does indeed occur in the insulating phase. At large exit slit sizes, a broadening of the Ru-peaks and the leading edge is observed, particularly in the yellow curve at 150~$\mu$m. However, by using a small enough exit slit size, the effect is minimal and does not change the overall features observed in the spectra. 

To verify that the charge gap is not influenced by sample aging, we measured the valence band spectrum immediately after, and a week after cleaving the crystal, shown in Fig.~\ref{sup4}b. Although there are some changes in the peak heights, the position of the leading edge remained the same. Note, the sample on which the aging spectra were taken was run through four iterations of current ramping up and down, thus the effect of constantly undergoing an IMT in the sample should be taken into account.

\section{transport-ARPES}\label{secA3}

\begin{figure}[h]%
\centering
\includegraphics[width=0.999\textwidth]{CoreLevels.pdf}
\caption{Sample fitting of core levels for the (a) S, (b) S*, (c) L-phases, and (d) S-phase post current. The individual Voigt and Gaussian peaks are shown in purple, the total fit in gray, and the raw data in black.}\label{sup6}
\end{figure}

Energy shifts are accounted for in this work using the Ca $3p$ and O $2s$ core level energies as reference points. An example of the core level fits is demonstrated in Fig.~\ref{sup6}. For all fits, a linear background is set and a Gaussian curve is used for the oxygen $2s$ peak, while two spin-orbit split Voigt curves are fitted to the calcium core level to account for a surface and bulk contribution. CRO typically cleaves between the RuO$_6$ layers, leaving a surface arrangement of Ca atoms that differs from the bulk, leading to slight asymmetry in the core level peak. Each Voigt curve is composed of two spin-orbit split peaks of the $p_{\frac{1}{2}}$ and $p_{\frac{3}{2}}$ orbitals. The ratio of the peak amplitudes is maintained at 2:1 based on atomic physics, and the difference between the peak positions is taken to be 420~meV from~\citep{albert1977} and \cite{herman_atomic_1963}. We present the exact numerical fits in the chart below.

\begin{table}[h]
\begin{center}
\begin{minipage}{375pt}
\caption{Fitting parameters for core levels}\label{tab1}%
\begin{tabular}{@{}cccccccccc@{}}
\toprule
Phase & Bulk Ca & $\sigma_{b}$ & $\gamma_{b}$ & Surface Ca & $\gamma_{s}$ & $\gamma_{s}$ & Ca Fit & O Peak & $\gamma_{o}$ \\
\midrule
S & -24.508 & -0.491 & 0.571 & -23.868 & -7.778e-5 & 0.918 & -24.459 & -20.414 & 2.339 \\
S* & -19.999 & -0.533 & 0.622 & -19.28 & 3.608e-5 & 0.732 & -19.974 & -15.955 & 2.157\\
L* & -23.144 & 1.02 & 0.046 & -22.298 & -0.0024 & 0.963 & -22.993 & -18.892 & 2.351 \\
S\footnotemark[1] & -24.548 & -0.371 & 0.651 & -23.948 & -0.371 & 0.651 & -24.556 & -20.392 & 2.048 \\
\botrule
\end{tabular}
\footnotetext{Bulk Ca, Surface Ca, Ca Fit and O Peak refer to the position of the peaks in energy (eV).}
\footnotetext[1]{Data taken after current has been ramped back down to 0mA.}
\end{minipage}
\end{center}
\end{table} 

The motivation for considering energy shifts with core levels primarily comes from the equivalent-core approximation. In other words, unlike the electronic states of the valence band, the wave vector of core levels are taken to be much more localized, thus expected to change less in comparison to low energy spectra. Shifts in energy are typically associated with the valency of the measured element, as observed in cuprates~\cite{}, or in a modified local potential which comes from an altered arrangement of surrounding atoms. However, in the case of CRO, the valency of the Ca$^{2+}$ ion is not expected to change in valency through the IMT.

This leaves the changing local environment contribution to the energy shift as the primary concern of this method. Interestingly, while the position and shape of the surface and bulk contributions to the Ca $3p$ peak are relatively similar in the insulating phases with and without current (i.e. S and S*), in the current-induced metallic phase, the contribution of the high energy Ca peak is decreased. Due to the higher energy, we attribute this peak to the bulk contribution, and the lower energy peak to the surface. It is well-known that as CRO goes through the IMT, the RuO$_6$ octahedra will become less tilted and distorted, which indeed changes the local environment surrounding Ca$^{2+}$ ions in bulk. Given that the primary differences occur in the higher energy Ca core level peak, it is logical to attribute these differences to a slightly modified arrangement of ions in the metallic state.

Ultimately, the primary validation for attributing the shifts of the core levels to the electric potential is the fact that both the Ca $3p$ and O $2s$ levels shift together. A changing local environment for the Ca$^{2+}$ ions also results in a changing environment for the O ions and should lead to some relative shift between the two peaks, however the distance between these peaks does not change within our uncertainty of 100~meV between the S- and L*-phases. The electric potential generated by the applied current across the sample is therefore the only mechanism that could cause such a large, uniform shift across both core levels.

\begin{figure}[h]%
\centering
\includegraphics[width=0.999\textwidth]{sup5}
\caption{Constant energy maps at E$_\mathrm{B} = -0.5$~eV at (a) 0~mA, in the S-phase, and (d) 4~mA, in the S*-phase with current. (b, c) EDCs integrated along the (b) $\Gamma Y$ and (c) $XM$ cuts showing minimal change aside from energy broadening caused by potential gradient across the beam spot. (e, f) MDCs integrated over 0.5~eV along (e) $\Gamma Y$ and (f) $XM$ showing slight inhomogeneity in the presence of current.}\label{sup5}
\end{figure}

An additional difficulty of transport-ARPES comes from inhomogeneous effects caused by stray magnetic fields. In order to assess inhomogeneous effects, we take cuts through data with and without current, as seen in Fig.~\ref{sup5}, and demonstrate that minimal change to the spectra, aside from shifts, occur. In order to correct for the the momentum shift, seen in Fig.~\ref{sup5}(a,d), we use the symmetry of the observed bands to determine the position of the $\Gamma$ point in the shifted spectral features, and thus, the shift of the momentum-space origin. Given that the momentum shift is tracked and corrected based on the observed symmetry of the spectral features, transport-ARPES is restricted to samples that are not too greatly influenced by matrix element effects such that obvious symmetry is hard to discern (e.g. CRO data taken with $\pi$-polarized light is hard to correct). Luckily, the symmetry of the band structure of most materials can be derived, in particular with high enough photon energy to capture the periodicity of the electronic structure.

\textit{The EDCs shown in Fig.~\ref{sup5}b and Fig.~\ref{sup5}c, taken through $\Gamma Y$ and $XM$ respectively, have been corrected for the energy shift to allow for comparison. The shapes of the EDCs further confirm that a broadening of about 100~meV of the spectra occurs with applied current.}\textcolor{red}{I don't see a broadening there, but rather a shift of the peaks. Am I misunderstanding something?}

On the other hand, spectral features that were equally intense without current, exhibit an asymmetry in intensity with current, as shown by the MDCs in Fig.~\ref{sup5}e and f. Note, these MDCs have been shifted in $k$ to allow for direct comparison, however the unshifted image is shown by the constant energy surface in Fig.~\ref{sup5}d. Momentum shifts are accounted for based on the symmetry of the features as discussed above. While the asymmetry is notable, it does not seem to change the overall appearance of features analysed in the data.

\section{DMFT Calculations}\label{secA4}

\begin{figure}[h]%
\centering
\includegraphics[width=0.69\textwidth]{DMFT.pdf}
\caption{DMFT calculations for the low energy Ru-bands in the (a, b) S-phase and (c, d) L*-phase.}\label{DMFT}
\end{figure}

The full set of DMFT calculations is displayed in Fig.~\ref{DMFT}. As mentioned in the main text, while the dispersion of the Ru bands are different along the $XM$ and $YM$ high-symmetry cuts, the calculated dispersions are qualitatively the same in both S- and L*-phases. While the calculations use the orthorhombic structural parameters of each phase, the orthorhombicity appears to have a much stronger influence in the experiment.

\section{Reproducibility}\label{secA5}

\begin{figure}[h]%
\centering
\includegraphics[width=0.999\textwidth]{reproducibility.pdf}
\caption{(a) I-V curve over multiple iterations. M-X-M cut for the sample reported in the main text (b) without and (c) with current after four rounds of ramping current up and down. The increased spectral weight at the X point and disappearance of spectral weight at $k^* = \pm 0.38$~\AA$^{-1}$ are still present in the current-induced bands, however the spectra much patchier. (d) EDC comparison with (black) and without (yellow) current. (e) I-V curve for a "bad" sample, i.e. a sample where smooth transport is not exhibited. X-M-X cuts (f) without and (g) with current, again, showing current-induced changes in patchy spectra.}\label{sup8}
\end{figure}

%\begin{figure}[h]%
%\centering
%\includegraphics[width=0.999\textwidth]{sup8}
%\caption{(a) $I$-$V$ curve over multiple iterations. $XM$ cut for the sample reported in the main text (b) without and (c) with current after four rounds of ramping current up and down. The increased spectral weight at the $X$ point and disappearance of spectral weight at $k_x = \pm 0.38$~\AA$^{-1}$ are still present in the current-induced bands, however the spectra much patchier. (d) EDC comparison with (black) and without (yellow) current. (e) $I$-$V$ curve for a "bad" sample, i.e. a sample where smooth transport is not exhibited. $XM$ cuts (f) without and (g) with current, again, showing current-induced changes in patchy spectra.}\label{sup8}
%\end{figure}

Upon removing the current, the equilibrium electronic structure is ``fully restored". However, as reported by Mattoni et al. \cite{mattoni2020} macroscopic cracks and defects will form during repeated cycles of the current-driven IMT. This is noticeable in the decrease of the maximum voltage of the IV curves reported in Fig.~\ref{sup8}. With a fast ramping of current to high magnitudes, the formation of these cracks are more likely to occur, causing a large dissipation of power as the resistance around these cracks will vary greatly. Despite conducting the experiment in UHV, overrunning power will cause a spark to occur, as demonstrated in the supplementary video.

While slow and careful ramping of the current allows one to do experiments over and over so long as the crystal has not broken, a spatial map after each new cycle of current must be taken to ensure that measurements are indeed done on a section of the crystal that the current is running through. A small beam spot is ultimately necessary in order to resolve where to avoid current-induced fissures, as well as the ``hot spots" that drive metallic phase formation/higher power dissipation reported by Mattoni et al. that grow as the result of current cycling. A more homogeneous current flow can also be provided if attaching electrical leads over the width of the sample as discussed in \cite{mattoni2020}. In other words, this experiment is reproducible so long as the current is ramped slowly and potential maps are methodically taken to ensure that photoemission data is indeed taken on an area with current running through it. 

\section{High temperature spectra}\label{secA6}

\begin{figure}[h]%
\centering
\includegraphics[width=0.999\textwidth]{highT.pdf}
\caption{Measurements taken at $T = 384$~K. (a) Fermi surface at 74~eV, integrated over $\pm 75$~meV. (d) DMFT simulated high temperature metallic Fermi surface. (b) DMFT computations along the high symmetry $XM$ and $YM$ cuts. Note, both cuts have the same dispersion. (e) $XM$ high symmetry cut taken from data. (f) High temperature EDC in red for the $XM$ cut integrated within the Brillouin zone compared with the current-induced EDC in purple from Fig.~\ref{fig3}b. (c) High temperature Fermi surface taken at 120~eV, integrated over $\pm 75$~meV. (g) $T=180$~K constant energy contour, taken at $E_{B} = -0.5$~eV, integrated over $\pm 50$~meV, for comparison. Note, at low temperatures, there are no spectral features at Fermi energy, thus this is the constant energy contour taken where spectral weight first starts to appear.}
\label{highT}
\end{figure}

The complete set of data taken at T = 384K is shown in Fig.~\ref{highT}. As discussed in the main text, the Fermi surface shown in Fig.~\ref{highT}a is markedly different from either current-induced Fermi surfaces. Unlike the current-induced DMFT, the high temperature experimental data does not appear to be in good agreement with the calculations shown in Fig.~\ref{highT}b. The most noticeable difference is the lack of high intensity features around the M points, which is also what most differentiates the high temperature Fermi surface from the current-induced Fermi surfaces. However, increase and decrease of spectral weight at the X and $k^* = \pm 0.38$~\AA$^{-1}$, respectively, along the $XM$-cut are present. This is highlighted by the shape of the EDCs between the high temperature (red) and current-induced (purple) phases displayed in Fig.~\ref{highT}f. Note, the high temperature EDC has an puturn above Fermi level, confirming the occupation of states in the metallic phase~\cite{•}. Finally, to highlight the difference between the high and low temperature data, we show constant energy contours taken at a photon energy of 120eV at T = 384K, $E_{F} = 0eV$ in Fig.~\ref{highT}c and T = 180K, $E_{B} = -0.5eV$ in Fig.~\ref{highT}g. At low temperatures, the spectral features closest to the Fermi level appear as a diamond-shape hugging the $\Gamma$-point. This diamond appears to expand in the high temperature phase.

\section{Notes on data displayed in the main text}\label{secA7}

\begin{figure}[h]%
\centering
\includegraphics[width=0.999\textwidth]{Fig3newdata.pdf}
\caption{Change in the Ru-band dispersion at $XM$ after four iterations of ramping current up and down. a) MDCs integrated over the energy range shown in the black (S) and yellow (L*) dashed boxes of the energy vs. momentum plots for the (b) S- and (c) L*-phases. (d,e) EDCs around (d) $X$ point and (e) $k^* = \pm 0.38$~\AA$^{-1}$ along the $XM$ line, highlighting the increase and decrease of spectral weight observed at the two $k$-points, respectively. Note, the effects are much less pronounced compared to Fig.~\ref{fig3}d and e, due to the fact that the crystal has deteriorated after four iterations of cycling the IV-curve, i.e. current no longer runs as smoothly through the crystal. The curves were obtained by integrating the photoemission intensity over the grey (0.26~\AA$^{-1}$) and purple 0.19~\AA$^{-1}$ box, respectively. (f,g) DMFT calculations for the (f) S- and (g) L*-phases.}
\label{newdata}
\end{figure}


Due to the difficulty of the experiment, all energy vs. momentum plots shown are taken from an experimental round where an incomplete set of core levels were taken, i.e. not all energies could be correctly calibrated. However, an additional experimental round was carried out where great care was taken to measure core levels before each spectrum, in addition to remaining at the same spot on the sample, such that the correct current-induced energy shifts could be obtained. Unfortunately during that experimental round, we could not measure with the same statistics. All EDCs, \textit{except for Fig.~\ref{fig3}d and e and Fig.~\ref{fig4}d and e} where EDCs are used to emphasize the difference in qualitative features, are taken from the energy-corrected experimental round. This include the EDCs and core levels, as well as the maps shown in Fig.~\ref{fig1} which are used to model the energy correction process. All current-induced energy vs. momentum plots were then shifted to the empirical binding energy is determined from the energy-corrected set. The same applies for the Fermi surfaces displayed in Fig.~\ref{fig2}a and Fig.~\ref{fig4}f. We present Fig.~\ref{newdata} with data from the energy-correct experimental round above to show that the discussed changes in band structure in the text are real. Note, these changes are also seen in Fig.~\ref{sup8}c from appendix ~\ref{secA5}, though the qualitative differences in dispersion are not as clear, like for the energy-correct sample set, due to internal cracks and fissures in the sample. All data is available online for further comparisons.

\end{appendices}


==> sn-bibliography.tex <==
\begin{thebibliography}{9}

@article{bertinshaw2019,
  author		= "Bertinshaw, J. and Gurung, N. and Jorba, P. and Liu, H. and Schmid, M. and Mantadakis, D. T. and Daghofer, M. and Krautloher, M. and Jain, A. and Ryu, G. H. and Fabelo, O. and Hansmann, P. and Khaliullin, G. and Pfleiderer, C. and Keimer, B. and Kim, B. J.",
  title			= "Unique Crystal Structure of ${\mathrm{Ca}}_{2}{\mathrm{RuO}}_{4}$ in the Current Stabilized Semimetallic State",
  journal		= "Phys. Rev. Lett.",
  volume		= "123",
  pages			= "137204",
  year			= "2019",
  doi			= "10.1103/PhysRevLett.123.137204"
}

@article{jain2017,
	author = "Jain, A. and Krautloher, M. and Porras, J. and Ryu, G. H. and Chen, D. P. and Abernathy, D. L. and Park, J. T. and Ivanov, A. and Chaloupka, J. and Khaliullin, G. and Keimer, B. and Kim, B. J.",
	doi = "10.1038/nphys4077",
	journal = "Nature Physics",
	pages = "633--637",
	title = "Higgs mode and its decay in a two-dimensional antiferromagnet",
	volume = "13",
	year = "2017"
}
	
@article{khaliullin2013,
  title = "Excitonic Magnetism in Van Vleck--type ${d}^{4}$ Mott Insulators",
  author = "Khaliullin, Giniyat",
  journal = "Phys. Rev. Lett.",
  volume = "111",
  pages = "197201",
  year = "2013",
  doi = "10.1103/PhysRevLett.111.197201"
}

@article{okazaki2013,
author = "Okazaki, R. and Nishina, Y. and Yasui, Y. and Nakamura, F. and Suzuki, T. and Terasaki, I.},
title = "Current-Induced Gap Suppression in the Mott Insulator Ca2RuO4",
journal = "Journal of the Physical Society of Japan",
volume = "82",
pages = "103702",
year = "2013",
doi = "10.7566/JPSJ.82.103702"
}


@article{ricco2018,
	author = "Ricc{\`o}, S. and Kim, M. and Tamai, A. and McKeown Walker, S. and Bruno, F. Y. and Cucchi, I. and Cappelli, E. and Besnard, C. and Kim, T. K. and Dudin, P. and Hoesch, M. and Gutmann, M. J. and Georges, A. and Perry, R. S. and Baumberger, F.",
	journal = "Nature Communications",
	pages = "4535",
	title = "In situ strain tuning of the metal-insulator-transition of Ca2RuO4 in angle-resolved photoemission experiments",
	volume = "9",
	year = "2018"
}

@article{braden1998,
  title = "Crystal and magnetic structure of ${\mathrm{Ca}}_{2}{\mathrm{RuO}}_{4}:$ Magnetoelastic coupling and the metal-insulator transition",
  author = "Braden, M. and Andr\'e, G. and Nakatsuji, S. and Maeno, Y.",
  journal = "Phys. Rev. B",
  volume = "58",
  pages = "847--861",
  year = "1998",
  doi = "10.1103/PhysRevB.58.847"
}

@article{alexander1999,
  title = "Destruction of the Mott insulating ground state of ${\mathrm{Ca}}_{2}{\mathrm{RuO}}_{4}$ by a structural transition",
  author = "Alexander, C. S. and Cao, G. and Dobrosavljevic, V. and McCall, S. and Crow, J. E. and Lochner, E. and Guertin, R. P.",
  journal = "Phys. Rev. B",
  volume = "60",
  pages = "R8422--R8425",
  year = "1999",
  doi = "10.1103/PhysRevB.60.R8422"
}

@article{steffens2005,
  title = "High-pressure diffraction studies on ${\mathrm{Ca}}_{2}{\mathrm{RuO}}_{4}$",
  author = "Steffens, P. and Friedt, O. and Alireza, P. and Marshall, W. G. and Schmidt, W. and Nakamura, F. and Nakatsuji, S. and Maeno, Y. and Lengsdorf, R. and Abd-Elmeguid, M. M. and Braden, M.",
  journal = "Phys. Rev. B",
  volume = "72",
  pages = "094104",
  year = "2005",
  doi = "10.1103/PhysRevB.72.094104"
}

@article{nakamura2013,
	author = "Nakamura, F. and Sakaki, M. and Yamanaka, Y. and Tamaru, S. and Suzuki, T. and Maeno, Y.",
	doi = "10.1038/srep02536",
	journal = "Scientific Reports",
	pages = "2536",
	title = "Electric-field-induced metal maintained by current of the Mott insulator Ca2RuO4",
	volume = "3",
	year = "2013"
}

@article{nakamura2002,
  title = "From Mott insulator to ferromagnetic metal: A pressure study of ${\mathrm{Ca}}_{2}{\mathrm{RuO}}_{4}$",
  author = "Nakamura, F. and Goko, T. and Ito, M. and Fujita, T. and Nakatsuji, S. and Fukazawa, H. and Maeno, Y. and Alireza, P. and Forsythe, D. and Julian, S.R.",
  journal = "Phys. Rev. B",
  volume = "65",
  pages = "220402",
  year = "2002",
  doi = "10.1103/PhysRevB.65.220402"
}

@article{dietl2018,
author = "Dietl,C.  and Sinha,S. K.  and Christiani,G.  and Khaydukov,Y.  and Keller,T.  and Putzky,D.  and Ibrahimkutty,S.  and Wochner,P.  and Logvenov,G.  and van Aken,P. A.  and Kim,B. J.  and Keimer,B.",
title = "Tailoring the electronic properties of Ca2RuO4 via epitaxial strain",
journal = "Applied Physics Letters",
volume = "112",
pages = "031902",
year = "2018",
doi = "10.1063/1.5007680"
}

@article{das2018,
  title = "Spin-Orbital Excitations in ${\mathrm{Ca}}_{2}{\mathrm{RuO}}_{4}$ Revealed by Resonant Inelastic X-Ray Scattering",
  author = "Das, L. and Forte, F. and Fittipaldi, R. and Fatuzzo, C. G. and Granata, V. and Ivashko, O. and Horio, M. and Schindler, F. and Dantz, M. and Tseng, Yi and McNally, D. E. and R\o{}nnow, H. M. and Wan, W. and Christensen, N. B. and Pelliciari, J. and Olalde-Velasco, P. and Kikugawa, N. and Neupert, T. and Vecchione, A. and Schmitt, T. and Cuoco, M. and Chang, J.",
  journal = "Phys. Rev. X",
  volume = "8",
  pages = "011048",
  year = "2018",
  doi = "10.1103/PhysRevX.8.011048"
}

@article{fuersich2019,
  title = "Raman scattering from current-stabilized nonequilibrium phases in ${\mathrm{Ca}}_{2}{\mathrm{RuO}}_{4}$",
  author = "F\"ursich, K. and Bertinshaw, J. and Butler, P. and Krautloher, M. and Minola, M. and Keimer, B.",
  journal = "Phys. Rev. B",
  volume = "100",
  pages = "081101",
  year = "2019",
  doi = "10.1103/PhysRevB.100.081101"
}

@article{zhang2019,
  title = "Nano-Resolved Current-Induced Insulator-Metal Transition in the Mott Insulator ${\mathrm{Ca}}_{2}{\mathrm{RuO}}_{4}$",
  author = "Zhang, J. and McLeod, A. S. and Han, Q. and Chen, X. and Bechtel, H. A. and Yao, Z. and Gilbert Corder, S. N. and Ciavatti, T. and Tao, T. H. and Aronson, M. and Carr, G. L. and Martin, M. C. and Sow, C. and Yonezawa, S. and Nakamura, F. and Terasaki, I. and Basov, D. N. and Millis, A. J. and Maeno, Y. and Liu, M.",
  journal = "Phys. Rev. X",
  volume = "9",
  pages = "011032",
  year = "2019",
  doi = "10.1103/PhysRevX.9.011032"
}

@article{mattoni2020,
  title = "Role of local temperature in the current-driven metal--insulator transition of ${\mathrm{Ca}}_{2}{\mathrm{RuO}}_{4}$",
  author = "Mattoni, G. and Yonezawa, S. and Nakamura, F. and Maeno, Y.",
  journal = "Phys. Rev. Materials",
  volume = "4",
  pages = "114414",
  year = "2020",
  doi = "10.1103/PhysRevMaterials.4.114414"
}

@article{albert1977,
  title = {Electronic band structure of fluorite},
  author = {Albert, J. P. and Jouanin, C. and Gout, C.},
  journal = {Phys. Rev. B},
  volume = {16},
  issue = {2},
  pages = {925--933},
  numpages = {0},
  year = {1977},
  month = {Jul},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevB.16.925},
  url = {https://link.aps.org/doi/10.1103/PhysRevB.16.925}
}

\end{thebibliography}


